Rare Yet Popular: Evidence and Implications from Labeled Datasets for Network Anomaly Detection

Anomaly detection research works generally propose algorithms or end-to-end systems that are designed to automatically discover outliers in a dataset or a stream. While literature abounds concerning algorithms or the definition of metrics for better evaluation, the quality of the ground truth against which they are evaluated is seldom questioned. In this paper, we present a systematic analysis of available public (and additionally our private) ground truth for anomaly detection in the context of network environments, where data is intrinsically temporal, multivariate and, in particular, exhibits spatial properties, which, to the best of our knowledge, we are the first to explore. Our analysis reveals that, while anomalies are, by definition, temporally rare events, their spatial characterization clearly shows some type of anomalies are significantly more popular than others. We find that simple clustering can reduce the need for human labeling by a factor of 2x-10x, that we are first to quantitatively analyze in the wild.

==> 90_appx.tex <==
\definecolor{appx}{gray}{0.9}
\input{table_clusters_smd}
\input{table_clusters_router}
 
%\section{Appendix}\label{sec:appx}
\appendix

We report for reproducibility (resp. completeness) detailed information concerning the top-10 Proximus clusters for the SMD (resp. Router) data sources in Tab.~\ref{tab:appx:smd} (resp. Tab.~\ref{tab:appx:router}). 
 Tables detail information about: the cluster rank, cluster size (individual and cumulated), dominant pattern and mean dispersion, spatial KPI footprint (quartiles and percentage of univariate events) and temporal duration of the anomaly (quartiles and percentage of spike events).
 
 
We also detail that the expert labelling exhibits patterns that would not appear for randomly generated data, following Sec.~\ref{sec:spatial_footprint} \AH{(not mentioned there currently)}.
Assuming two events generated by taking randomly $A$ anomalous KPIs among $F$ KPIs, the number of shared KPIs $l$ verifies:
\begin{align}
\mathbb{P}(l = F) = \binom{A}{l} \binom{F-A}{A-l} \bigg/ \binom{F}{A},
\end{align}
giving an expected number $\mathbb{E}(l) =\sum_{l=0}^{F} l P(l) = A^2/F$ of shared KPIs. %$l$ is:
\begin{align}
\mathbb{E}[l] = \sum_{l=0}^{F} l P(l) = \sum_{l=0}^{F} l \binom{A}{l} \binom{F-A}{A-l} \bigg/ \binom{F}{A} = A^2/F.
\end{align}
Numerically, taking $A=4$ (median number of anomalous KPIs for both Router and SMD) and either $F=87$ (Router) or $F=38$ (SMD), we expect less than one KPI in common.
Observing large groups of spatial clusters indicates that the labeling follows several patterns that would not appear using randomly generated data. \AH{but for our data we also observe a small intersection in average: commonly the intersection is 0 because the 2 events of the labels would be in different clusters} \AH{We could compare the values 0.42, 0.18 with the intersection observed in the clusters after applying Proximus, which is probably greater than 1}   performed by the expert is exhibiting a semantically relevant structure.

% # Router
% F = 87 # median number of KPIs
% A = 4 # median number of anomalous KPIs
% A^2/F # 0.18 = expected number of matches for A randomly anomalous among F
% # SMD
% F = 38 # median number of KPIs
% A = 4 # median number of anomalous KPIs
% A^2/F # 0.42 = expected number of matches for A randomly anomalous among F
% # Both are < 1, so if they were randomly generated we wouldn't expect clusters



==> table_clusters_router.tex <==
\begin{table*}[!t]
\caption{Detailed summary of Router top-10 Proximus clusters (obtained with $ R^+=6, S^-=8$)}\label{tab:appx:router}
\centering
\begin{tabular}{rcccccc}
\toprule
\textbf{Cluster}       & \textbf{\% Samples} & \textbf{\begin{tabular}[c]{@{}c@{}}Cumulative\\ \% Samples\end{tabular}} & \textbf{Dominant Pattern}                                                            & \textbf{\begin{tabular}[c]{@{}c@{}}Mean \\ Dispersion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}KPIs \\ (min, Q1, median, Q3,\\  max, \% univariate)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Duration \\ (min,Q1, median, Q3,\\  max, \% spike)\end{tabular}} \\ 
\midrule
\rowcolor{appx}
\multicolumn{1}{c}{1} & 45.7\%  & 45.7\%  & \begin{tabular}[c]{@{}c@{}}\{cause i nhlfe invalid,\\  excp ID l2 mplsuc\}\end{tabular}  & 1.0 & (1, 2, 2, 2, 32, 3.8\%) & (1, 1, 1, 1, 213, 77.5\%) \\ %\cline{2-7} 
\multicolumn{1}{c}{2} & 7.4\%  & 53.1\%  & \begin{tabular}[c]{@{}c@{}}\{cause drop ecar red,\\ cause cpu ipv4 ttl err\}\end{tabular} & 2.5 & (1, 2, 2, 5, 18, 7.7\%) & (1, 1, 2, 19, 162, 38.5\%) \\ %\cline{2-7} 
\rowcolor{appx}
\multicolumn{1}{c}{3} & 6.9\% & 60\% & \{cause\_e\_fhparse\_aib\_invalid\} & 0.2 & (1, 3, 3, 3, 22, 8.3\%) & (2, 2, 3, 3, 4, 0\%) \\ %\cline{2-7} 
\multicolumn{1}{c}{4} & 5.7\% & 65.7\% & \{cause\_cpu\_fib\_miss\} & 0.4 & (1, 2, 3, 7, 8, 10\%) & (1, 2, 3, 3, 4, 10\%) \\ %\cline{2-7} 
\rowcolor{appx}
\multicolumn{1}{c}{5} & 4.8\% & 70.5\% & \{cause\_i\_l2i\_pat\_inv\} & 0 & (1, 1, 1, 1, 1, 100\%) & (1, 1, 1, 1, 2, 87.5\%) \\ %\cline{2-7}
 
\multicolumn{1}{c}{6} & 4.6\% & 75.1\% & \{excp\_id\_ipv4\_fib\_miss\} & 1.3 & (1, 1, 2, 2, 12, 37.5\%) & (1, 2, 13, 147, 519, 12.5\%) \\ %\cline{2-7}
\rowcolor{appx}
\multicolumn{1}{c}{7} & 4.0\% & 79.1\% & \{drop\_excp\_id\_ipv4\_ttl expired\} & 0 & (2, 4, 4, 4, 10, 100\%) & (1, 4, 5, 7, 10, 14.3\%) \\ %\cline{2-7}
\multicolumn{1}{c}{8} & 2.3\% & 81.4\% & \begin{tabular}[c]{@{}c@{}}\{drop\_id\_qvct\_miss\_no\_dhcp\_req\_no\_arp,\\ cause\_cpu\_ipv4\_tunnel\_end\}\end{tabular} & 0.8 & (1, 1, 1, 1, 2, 75\%) & (1, 4, 6, 74, 281, 25\%) \\ %\cline{2-7}
\rowcolor{appx}
\multicolumn{1}{c}{9} & 2.3\% & 83.7\% & \{excp\_id\_mpls\_ttl\_expired\_discard\} & 0 & (1, 1, 1, 1, 1, 100\%) & (1, 1, 1, 1, 1, 100\%) \\ %\cline{2-7}
\multicolumn{1}{c}{10} & 1.7\% & 85.4\% & \{excp\_id\_l2\_mplsuc\_discard\} & 0 & (1, 1, 1, 1, 1, 100\%) & (1, 1, 1, 1, 1, 100\%)\\
\bottomrule
\end{tabular}
\end{table*}

==> table_clusters_smd.tex <==
\begin{table*}[!t]
\caption{Detailed summary of SMD top-10 Proximus clusters (obtained with $ R^+=29, S^-=12$)}\label{tab:appx:smd}
\centering
\begin{tabular}{rcccccc}
\toprule

\textbf{Cluster}       & \textbf{\% Samples} & \textbf{\begin{tabular}[c]{@{}c@{}}Cumulative\\ \% Samples\end{tabular}} & \textbf{Dominant Pattern}                                                                                                                 & \textbf{\begin{tabular}[c]{@{}c@{}}Mean \\ Dispersion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}KPIs \\ (min, Q1, median, Q3,\\  max, \% univariate)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Duration \\ (min,Q1, median, Q3,\\  max, \% spike)\end{tabular}} \\ 
\midrule
\rowcolor{appx}
\multicolumn{1}{c}{1} & 35.4\%  & 35.4\% & \begin{tabular}[c]{@{}c@{}}\{disk\_svc, disk\_u, disk\_q,\\ disk\_wa, disk\_w\}\end{tabular} & 5.2 & (3, 4, 5, 8, 34, 0\%) & (2, 4, 10, 148, 3161, 24.3\%) \\ %\cline{2-7} 
\multicolumn{1}{c}{2} & 18.2\%  & 53.6\% & \{disk\_r, disk\_u, disk\_rb\} & 4.4  & (2, 4, 4, 7, 23, 0\%) & (3, 3, 5, 23, 872, 37.3\%) \\ %\cline{2-7} 
\rowcolor{appx}
\multicolumn{1}{c}{3} & 11.7\% & 65.3\% & \begin{tabular}[c]{@{}c@{}}\{cpu\_r, eth1\_fi, eth1\_fo,\\ eth1\_pi, eth1\_po, in\_segs,\\ out\_segs, tcp\_tw,\\ active\_opens\}\end{tabular} & 5.9  & (5, 10, 12, 14, 21, 0\%) & (3, 21, 33, 95, 573, 2.6\%) \\ %\cline{2-7} 
\multicolumn{1}{c}{4} & 6.5\% & 71.8\% & \{disk\_svc, disk\_wa\} & 0.8 & (1, 2, 2, 2, 3, 9.5\%) & (3, 8, 32, 53, 225, 19\%) \\ %\cline{2-7} 
\rowcolor{appx}
\multicolumn{1}{c}{5} & 5.5\% & 77.3\% & \begin{tabular}[c]{@{}c@{}}\{retransegs,\\ tcp\_timeouts\}\end{tabular}  & 1.1 & (2, 2, 3, 3, 8, 0\%) & (3, 4, 5, 50, 131, 16.7\%) \\ %cline{2-7}
 
\multicolumn{1}{c}{6} & 3.7\% & 81.0\% & \begin{tabular}[c]{@{}c@{}}\{udp\_out\_dg, cpu\_r, \\ load\_1, load\_5, load\_15, \\ mem\_u, retransegs, \\ tcpu\_timeouts, disk\_wb, \\ eth1\_fi, eth1\_fo, \\ eth1\_pi, eth1\_po, \\ curr\_estab, in\_segs, \\ out\_rsts, out\_segs, \\ passive\_opens, mem\_u\_e,\\ udp\_in\_dg, tcp\_tw, \\ tcp\_use, active\_opens\}\end{tabular}  & 5.1 & (15, 18, 20, 21, 25, 0\%) & (11, 57, 89, 205, 305, 0\%) \\ %cline{2-7}
\rowcolor{appx}
\multicolumn{1}{c}{7} & 3.7\% & 84.7\% & \begin{tabular}[c]{@{}c@{}}\{cpu\_r, load\_1,\\ load\_5, load\_15, \\ mem\_u, curr\_estab, \\ mem\_u\_e, tcp\_use\}\end{tabular}  & 3.8 & (4, 6, 8, 8, 14, 0\%) & (10, 16, 27, 80, 786, 0\%) \\ %cline{2-7}
\multicolumn{1}{c}{8} & 3.1\% & 87.8\% & \{disk\_q\} & 2.3 & (2, 2, 2, 3, 10, 0\%) & (3, 3, 19, 157, 452, 40\%) \\ %cline{2-7}
\rowcolor{appx}
\multicolumn{1}{c}{9} & 2.8\% & 90.6\% &\{out\_rsts\}  & 0.8 & (1, 1, 1, 1, 2, 88.9\%) & (3, 3, 3, 5, 76, 55.6\%) \\ %cline{2-7}
\multicolumn{1}{c}{10} & 2.2\% & 92.8\% & \begin{tabular}[c]{@{}c@{}}\{mem\_u, disk\_rb\\ disk\_wb, mem\_u\_e\}\end{tabular}  & 1.6 & (2, 3, 4, 4, 6, 0\%) & (3, 3, 4, 13, 36, 28.6\%)\\
\bottomrule
\end{tabular}
\end{table*}
